When to Show a Suggestion? Integrating Human Feedback in AI-Assisted Programming

AI powered code-recommendation systems, such as Copilot and CodeWhisperer, provide code suggestions inside a programmer's environment (e.g., an IDE) with the aim of improving productivity. We pursue mechanisms for leveraging signals about programmers' acceptance and rejection of code suggestions to guide recommendations. We harness data drawn from interactions with GitHub Copilot, a system used by millions of programmers, to develop interventions that can save time for programmers. We introduce a utility-theoretic framework to drive decisions about suggestions to display versus withhold. The approach, conditional suggestion display from human feedback (CDHF), relies on a cascade of models that provide the likelihood that recommended code will be accepted. These likelihoods are used to selectively hide suggestions, reducing both latency and programmer verification time. Using data from 535 programmers, we perform a retrospective evaluation of CDHF and show that we can avoid displaying a significant fraction of suggestions that would have been rejected. We further demonstrate the importance of incorporating the programmer's latent unobserved state in decisions about when to display suggestions through an ablation study. Finally, we showcase how using suggestion acceptance as a reward signal for guiding the display of suggestions can lead to suggestions of reduced quality, indicating an unexpected pitfall.

==> new_body.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




Code recommendation systems powered by large-scale neural language models such as  Github Copilot \cite{copilot} and  Amazon CodeWhisperer \cite{codwhisperer} provide programmers with code suggestions to help improve their productivity. The usual way these systems operate is by displaying the suggestion as {\em ghost text} -- a greyed-out code suggestion inline inside the IDE. The programmer can then accept the suggestion, browse through different suggestions or reject the suggestion; this is illustrated in Figure~\ref{fig:ide_coderec}. The code suggestions appear either at the explicit invocation of the programmer or when the programmer pauses their cursor when writing code. A recent study from GitHub, which performed a randomized study with 95 participants who wrote a web server, 
found that Copilot could potentially reduce task completion time by a factor of two {\cite{kalliamvakou_2022}}. 
This provides evidence that these systems can already improve programmer productivity and motivates our research to pursue potential improvements to these systems.

The backend of these systems is large language models (LLMs) such as GPT which are trained on standard language modeling objectives using the Common Crawl data \cite{radford2019language}, and then fine-tuned on public code repositories \cite{chen2021evaluating}. The public roll-out of the code recommendation models has attracted millions of programmers, enabling a unique opportunity to leverage the data of programmers interacting with the models. In this work, we study GitHub's Copilot which is used by millions of programmers \cite{copilot}. For programmers within our organization who consented to have their usage data collected, we collected telemetry data of Copilot  suggestions with their associated prompts and the programmer's action to accept or reject the suggestions. We leverage this telemetry data to design interventions that improve the interaction between programmers and \coderec. 

Specifically, the first  question we wish to answer is \emph{when} to show a code suggestion.
We first define the notion of suggestion utility, a theoretical value that measures the impact of showing a suggestion on the overall time to write a specific piece of code, this value provides an optimal criteria for when to show a suggestion. However, computing suggestion utility is highly difficult and not currently feasible. Instead, we show that suggestion utility increases the more likely a suggestion is to be accepted and decreases with the latency to generate a suggestion, two quantities we can reliably estimate and control respectively. We develop an intuitive procedure named {\bf C}onditional Suggestion {\bf D}isplay from {\bf H}uman {\bf F}eedback (CDHF) which decides at each pause in keystrokes first whether it's worthwhile to generate a suggestion, if so then decides if the programmer is likely to reject the suggestion generated and either hides or shows the suggestion accordingly. 
The CDHF method is based on cascading models that predict acceptance of suggestions and can guarantee via its optimization procedure that any suggestion that was hidden (or not generated) would have been rejected if it was shown with a probability of at least $p$ where $p$ can be $0.99$. 

Using data from programming sessions of 535 programmers in our organization with feedback on 168k suggestions, we perform a retrospective evaluation of CDHF notably showing that we can hide 25\% of suggestions that were shown while guaranteeing that 95\% of them would have been rejected and avoiding to generate 13\% of these suggestions. This would lead to a hypothesized increase in the acceptance rate by  7.2\%. The CDHF procedure allows for a trade-off between the number of suggestions that are hidden and reducing latency by avoiding generating suggestions with a hyperparameter $\lambda$. We note that a minimal version of CDHF has been implemented in newer version of GitHub Copilot \cite{newcopilot2023} following the presentation of preliminary versions of our work to GitHub, however, our paper showcases how one can build better forms of suggestion display and this is still relevant. 

One may argue that the action of accepting or rejecting a suggestion may not always be fully indicative of programmer preference -- there may be a confounding context that drives these actions, notably what the programmer was doing/thinking at the time. We use this insight to motivate modeling the programmer's latent state of thought when building such predictive models of acceptance. Building on the literature in \cite{mozannar2022reading} that conducted a data collection study with 21 participants that included their latent state, we show that including latent state in predicting acceptance of suggestions leads to significantly better results and thus motivating collecting data beyond what is captured in telemetry. Finally, we investigate whether we can use suggestion acceptance as a reward signal to select \emph{which} suggestions to display and show that it can prioritize partial completions over complete code segments. While we investigate Copilot in this work, we believe our insights extend to other AI models and non-code-based tasks \footnote{Note: Some of the results in this paper were previously included in a separate paper \cite{mozannar2022reading}.}.

To summarize, we contribute: 

\begin{enumerate}
    \item A mathematical framework for AI-Assisted Programming named CDHF, that decides when to show code suggestions to save programmers time.
    \item A prediction model of the programmer's actions learned from hundreds of users to operationalize CDHF and save programmer time in AI-assisted programming with extensive evaluation including an analysis of factors that influence action predictions
    \item An experimental analysis of unintended consequences of ranking suggestions by probability of acceptance.
\end{enumerate}


% optional contribution bullet list

%The remainder of this paper is structured as follows: We first review related work on AI-assisted programming (Section \ref{sec:related_work}) and describe our problem setting in Section~\ref{sec:ai_programming}. We then introduce our utility theory formulation and understanding of the programmer's latent state in Section~\ref{sec:utility_theory} and our proposed method CDHF in Section~\ref{sec:cdhf} and finally our experimental results in Section~\ref{sec:experiments}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}\label{sec:related_work}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The closest related work to ours is the procedure to selectively hide  suggestions  in \cite{sun2022learning} (Quality Estimation Before Completion, QEBC). However, QEBC \cite{sun2022learning} is not based on human feedback of accepting suggestions, but rather is based on constructing a learned estimator of the quality of code completions from datasets of paired code segments and model completions. In contrast, our CDHF estimator uses real programmer behavior data and is based on data from a code-recommendation system in current use (Copilot) as opposed to custom-trained ones in \cite{sun2022learning}. %Codex, the underlying model of Copilot, was tested on the HumanEval dataset of 164 programming problems, where it was asked to write the function body from a docstring and achieved 37.7\% accuracy with a single generation \cite{chen2021evaluating}.
Different metrics and datasets have been proposed to evaluate the performance of code recommendation models, but these typically assess how well the model can complete code in an offline setting without developer input, rather than evaluating how well it assists programmers in-situ \cite{ziegler2022productivity,li2022competition,evtikhiev2022out, dakhel2022github}.
%Weisz et al. conducted interviews with developers and found that they did not require a perfect recommendation model for the model to be useful \cite{weisz2021perfection}. On the other hand, a study of 24 participants by Vaithilingam et al. showed no significant improvement in task completion time, yet participants stated a clear preference for Copilot \cite{vaithilingam2022expectation}. \cite{barke2022grounded} and \cite{mozannar2022reading} categorize programmer activities when interacting with Copilot.
Integrating human preference when training machine learning models have long been studied in the literature \cite{knox2008tamer,macglashan2017interactive}. In particular, Reinforcement Learning from Human Feedback has been used to improve LLMs as chat agents \cite{ziegler2019fine,bai2022training} notably including ChatGPT \cite{chatgpt}. In contrast, our approach CDHF uses organic human feedback through telemetry  which is not fully reflective of  preference and has an objective of fast inference to reduce latency and hiding suggestions rather than updating the LLM. Further related work can be found in Appendix. Our theoretical formulations build on earlier work on harnessing machine learning and utility to guide AI versus human-powered contributions in human-AI interactive settings \cite{horvitz1999principles}, which we apply to our setting.
%Work on algorithmic deferral %Our theoretical formulations in Section~\ref{sec:utility_theory} builds on the work of interactive user interfaces \cite{horvitz1999principles,dudley2018review} and generalize them to our setting. %Work on algorithmic deferral \cite{raghu2019algorithmic,okati2021differentiable} investigates a similar question on whether the human or the AI should accomplish the task and is based on error estimation (instead of time cost estimation here) of the human versus the AI, as well as work on  personalized decision support policies \cite{bhatt2023learning} investigates whether support should be shown but not when.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Problem Setting}\label{sec:ai_programming}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{\coderec.} We consider \coderec, which is a commonly used and exemplary tool of AI-powered code recommendations used by millions of programmers \cite{copilot}. \coderec is powered by a Large Language Model (LLM) and helps programmers within an IDE by providing code suggestions whenever the programmer pauses their typing. An illustration of \coderec suggesting code as an inline, single-colored snippet is shown in Figure~\ref{fig:ide_coderec}. The programmer can choose to accept this suggestion by utilizing a keyboard shortcut (e.g., tab).

\paragraph{AI-Assisted Programming.} We attempt a mathematical formalization of programming with the help of a code recommendation model such as \coderec which we dub \emph{AI-Assisted Programming}. The programmer wishes to complete a certain task $T$, for example, implement a logistic regression classifier that classifies 
\begin{comment}
We assume there are specific criteria that the programmer must meet for the task to be considered complete that are a function of the code and the task. This is meant to mimic software development tests, in our example, it might mean obtaining a test accuracy above 80\%, one may also consider a continuous criteria that takes into account time and sample complexity, security vulnerabilities, and task performance. We assume the programmer's \textbf{goal} is to complete the task to completion in a session while trying to minimize time spent completing the task. 
\end{comment}
As the programmer writes code  starting from  time  $0$, \coderec will attempt to provide code suggestions at different instances in time during the session. At a given time $t$, \coderec \footnote{We keep implementation details of Copilot to a high level, this work is based on the August 2022 version of Copilot.} uses a portion of the code $X_t$ to generate a prompt $P_t$, which is passed to the underlying LLM. \coderec then generates a code suggestion $S_t$ which will be shown to the user at time $t+\tau$ where $\tau$ accounts for the LLM latency.  Once the suggestion is shown, the programmer  must make an action at a certain time $t'>t+\tau$, the action is $A_{t'} \in \{\textrm{ accept, reject}\}$; the \emph{reject} action is triggered implicitly by continuing to type.  While the programmer's actions can be modeled as a continuous-time Markov Decision Process with the state space being the code $X$ which includes \coderec suggestions and the actions being writing code and acting on suggestions, we want to restrict our attention to the interaction between the programmer and \coderec which is captured via telemetry. 

\paragraph{Telemetry.} \coderec logs aspects of the interactions via {\em telemetry} which we leverage here, time is now discretized in terms of event positions to which we refer. 
Specifically, whenever a suggestion is shown, accepted or  rejected, we record a tuple to the telemetry database, $(t_i, A_i, P_i, S_i)$, where $t_i$ represents the within-session timestamp of the $i^\text{th}$ event ($t_0 = 0$), $A_i$ details the action taken (augmented to include `shown'), and $P_i$ and $S_i$ capture  the prompt and suggestion, respectively. Figure~\ref{fig:telemetry} displays the telemetry of a coding session. The telemetry stored in a database $D=\{(t_i, A_i, P_i, S_i)\}_{i=1}^n$ for each programmer, and represents a  discretized representation of the interaction and is the human feedback data we leverage.  


\begin{figure}[t]
	\centering
\includegraphics[width=0.5\textwidth]{figures/telemetry_short.pdf}
	\caption{Schematic of  telemetry with \coderec as a timeline. For a given coding session, the telemetry contains a sequence of timestamps and actions with associated prompts and suggestions.}
	\label{fig:telemetry}
\end{figure}

\textbf{Programmer State.} The telemetry does not capture the programmer's activities and thinking between two consecutive time stamps $t_i$ and $t_{i+1}$, i.e. the space in between the arrows in Figure~\ref{fig:telemetry} which we refer to as the programmer's latent state.
When faced with a suggestion, is the programmer looking and verifying it, or is the programmer engaged in other activities such as thinking about their code or looking at documentation? This is of critical importance, since from the point of view of the telemetry, two similar suggestions with similar prompts may have different programmer actions unbeknownst to us only because the programmer's latent state was different.  In this work, we try to understand the impact of the programmer latent state denoted as $\phi_t$ and its effect on our ability to leverage the telemetry (human feedback data) to improve AI-code recommendation systems. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Theoretical Formulation of Suggestion Utility}\label{sec:utility_theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


A critical design question in programmer-{\coderec} interaction is \textbf{when} should the model inject a suggestion into the IDE?
While the version of {\coderec} studied here provides a suggestion when it detects a brief pause in the IDE, an alternative is to not suggest and allow the programmer to ask for suggestions using a keyboard shortcut. However, the latter may lead to a sub-optimal interaction because its success would require the programmer to build a very accurate mental model of {\coderec} abilities {\cite{sarkar2022like}}, which is possible but only with lengthy interactions with the model \cite{bansal2019beyond} or with training \cite{mozannar2022teaching}. Second, requiring an
explicit invocation can disrupt the natural flow of programming, breaking a state of flow achieved during intensive focus {\cite{csikszentmihalyi2014flow}}. Designs requiring user initiative as well as those automatically displaying content can burden users with interruptions that decrease task performance \cite{bailey2001effects,Cutrell2001Interrupt}. We note that such costs can be inferred and accounted for formally in utility-theoretic systems \cite{HA_Interrupt2003,Attention_sensitive1999}. 

Ideally, {\coderec} should display suggestions when the suggestions provide value to programmers. For example, consider the task of completing a function and the time taken to complete it as a proxy for the overall effort. If the expected time required to verify and edit {\coderec}'s suggestion exceeds the time to write the code by themselves (counterfactual cost), then {\coderec} should not show its suggestions. Conversely, if the expected time to write exceeds the time to verify and edit, it may be useful to display the suggestion. We now formalize this intuition with a utility theoretical formulation and in the next section discuss the methodology to make it practical.  

\textbf{Programmer Model.} At a given time instance time during a session, \coderec extracts a prompt $P$ from the code file $X$ and generates a code suggestion $S$. If this suggestion is shown, we assume the programmer spends an expected time $\E[\mathrm{verification}|X,S,\phi]$ to verify it and follows a probability law $\bP(A=\textrm{accept}|X,S,\phi)$ to accept suggestions. 
Once a suggestion is accepted, the programmer may further edit the suggestion with expected time $\E[\mathrm{editing}|X,S,\phi,A=\mathrm{accept}]$ to  achieve their task. On the other hand, suppose the programmer rejects the suggestion, then they would have to spend time writing code that achieves their task and this is denoted by $\E[\mathrm{writing}|X,S, A=\mathrm{reject}]$. 
Thus the total time that showing a suggestion incurs is denoted as $\E[\mathrm{S \ shown}|X,S,\phi]$ is:
\begin{align}\label{eq:time_shown}
	&\E[\mathrm{S \ shown}|X,\phi] = \E[\mathrm{verification}|X,S,\phi] 
	\\&+ \bP(A=\textrm{accept}|X,S,\phi) \cdot  \E[\mathrm{editing}|X,S,\phi,A=\mathrm{accept}]  \nonumber\\
	&+\bP(A=\textrm{reject}|X,S,\phi) \cdot  \E[\mathrm{writing}|X,S, \phi, A=\mathrm{reject}] \nonumber
\end{align}

While editing and writing, \coderec may further make more suggestions thus the editing time and writing time should include interactions with future suggestions. 
Now on the other hand, if the suggestion is \emph{not} shown,  the programmer will spend time $\E[\mathrm{writing}|X]$ writing  code for their task.
We also need to factor in latency $\tau$ time cost to compute a suggestion once we decide to create a suggestion. Latency is only experienced by the programmer if they expect a suggestion and are waiting for it, which would be reflected in their latent state $\phi$. If the programmer is expecting a suggestion, we should add a time $\tau$ for latency to the total time when we show a suggestion, otherwise, the programmer continues to write code not expecting a suggestion. 


We now define the notion of suggestion utility, which is a numeric value that indicates the change in programmers coding time due to showing the suggestion.
\begin{definition}[Suggestion Utility]
	The time impact $\delta$, denoted as the \emph{suggestion utility}, of showing $S$ versus not showing is defined as:
	\begin{align}\label{eq:delta}
		&\delta =   
		\underbrace{\E[\mathrm{writing}|X,\phi]}_{\mathrm{S \ not \  shown}} - \underbrace{\E[\mathrm{S \ shown}|X,\phi]}_{\mathrm{S\ shown}}  - \underbrace{\E[\tau|X,\phi]}_{\mathrm{latency}}
	\end{align}
\end{definition}
From the above, a suggestion $S$ at a given time should \textbf{only be shown} if $\delta >0$ (Equation~\ref{eq:delta}), this would imply that the programmer will spend less time to achieve their task if it is shown.
An optimal scheme to know when to show suggestions would be to generate suggestions as frequently as possible and compute their \emph{suggestion utility} $\delta$ and show them if $\delta >0$.

\paragraph{Feasibility of Estimating $\delta$.} Equation \eqref{eq:time_shown} to compute \emph{suggestion utility} requires the computation of 4 different quantities: (1) the expected time spent verifying a suggestion, (2) the expected time editing a suggestion, (3) the expected time to write a segment of code and (4) the probability of accepting a suggestion. One can attempt to build an estimator for (1), by predicting from the  prompt and suggestion the time spent verifying a suggestion $i$ which would be $t_{i+1}-t_{i}$ using standard regression estimators. Unfortunately, using the same features and the dataset detailed in our experimental section, our best estimator was only able to achieve an $R^2=0.13$ which is not much better than a naive median time estimate. This might be due to the high variance and unobserved confounders governing verification time. Estimating editing and verification time (quantities 2 and 3 above) is only more complex and challenging and thus we restrict our methodology to seeing when can we evaluate $\delta$ using only our estimator for the probability of acceptance (4). 

\paragraph{Learning Programmer's Acceptance Decisions.} The full form for the probability that the programmer accepts a suggestion is $\bP(A=\textrm{accept}|X,S,\phi)$. Given the telemetry  one can only compute $\bP(A=\textrm{accept}|X,S)$ where the programmer latent state cannot be observed.  Using standard calibrated classification methods, we can estimate the probability $\bP(A=\textrm{accept}|X,S)$  by using the actions $A_i$ as the labels. 
We show that a simple mechanism  of thresholding the estimated probability that the programmer accepts a suggestion is equivalent under certain assumptions to checking if $\delta < 0$:
\begin{proposition}\label{prop:pstar}
	Under assumptions of the programmers model, notably that the programmer spends more time writing code when they reject a suggestion compared to when they accept a suggestion and edit it. Given  specific code, suggestion and latent state $(X,S,\phi)$, if the programmer's probability of accepting $\bP(A=\textrm{accept}|X,S,\phi)$ a suggestion is below $\bP^*$, which is defined as:
	\begin{align}\label{eq:p_star}
		& \bP^* = \frac{\E[\mathrm{verification}] + \E[\mathrm{latency}] }{   \E[\mathrm{writing}|A=\mathrm{reject}] - \E[\mathrm{editing}|A=\mathrm{accept}] } 
	\end{align}
	then the suggestion should not be shown. Note that $\bP^*$ is defined as a function $\bP^*(X,S,\phi)$ evaluated pointwise. 
\end{proposition}

The formal statement and proof are available in the appendix. The above proposition shows that comparing the probability of acceptance to $\bP^*$   can guide when to show the suggestion. We provide a graphical view of the analysis in Figure \ref{fig:pstar}, in the spirit of related analyses on utility-guided interactive interfaces \cite{horvitz1999principles}. Practically, if we compare the probability of acceptance to a constant lower bound of $\bP^*$, we can guarantee that we hide suggestions only when $\delta <0$.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.6\textwidth]{figures/pstar_fig.pdf}
	\caption{A visual depiction of Proposition \ref{prop:pstar} when the latency is zero. The y-axis indicates total time, the x-axis is  the programmer's probability of accepting $\bP(A=\textrm{accept}|X,S,\phi)$. The point $\bP^*$ is the one where showing or not showing the suggestion has equal time cost.   }
	\label{fig:pstar}
\end{figure}



\paragraph{Effect of Programmer Latent State.} As mentioned previously, the programmer's latent state is not included in the telemetry so we can only build the model $\bP(A=\textrm{accept}|X,S)$ compared to a model with the latent state $\bP(A=\textrm{accept}|X,S,\phi)$. \cite{mozannar2022reading} collected telemetry data of 21 programmers' performing various tasks and had participants retrospectively label the telemetry with their latent state from a set of twelve unique states (1096 suggestions). We use this data to build predictive models with and without the latent state using the same methodology in the experiments section \ref{sec:experiments}. Using a leave-one-out programmer evaluation strategy, the model without the latent state achieves accuracy $61.9 \pm 1.9$ while the model with the latent state achieves $83.6 \pm 2.4 $ which is a statistically significant difference according to a paired t-test ($p=6.9e-7,t=7.11$); a similar result occurs when comparing AUCs. This highlights an opportunity to gather external data beyond telemetry to build such models and indicates that acceptance may not simply  be a property of suggestions and code context.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conditional Suggestion Display From Human Feedback}\label{sec:cdhf}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we propose our Conditional suggestion Display from Human Feedback method that can be implemented using telemetry data to know when to show suggestions illustrated in Figure~\ref{fig:ide_coderec}.  Motivated by the prior section, we have seen that from equation \eqref{eq:p_star}  the higher the probability of accepting the suggestion and the lower the latency to generate the suggestion, the more likely the suggestion is useful ($\delta>0$). Our proposal is as follows: each time the programmer pauses typing, we decide using a predictor  whether to show a suggestion. Crucially, we do this using a two-stage scheme to avoid generating some of the suggestions when we know the programmer would reject them.  


\paragraph{Display Decision.} Let $m(X,S)$ be a binary predictor of the code and the suggestion that denotes whether at a given moment in the code $X$, we should show the suggestion $S$; we call this the display decision. If $m(X,S)=1$ we display the suggestion and otherwise do not.  
The most straightforward way to build such a function $m$ is to estimate the programmer's probability of accepting the suggestion: $\bP(A=\textrm{accept})|X,S)$ and then threshold the probability so that suggestions that fall below a probability $t$ are hidden. However, this will lead us to always generate suggestions when some of them will never be shown and thus wasting compute resources. We propose to decompose the function $m$ so that we first decide using  only the code whether we can make the display decision without generating the suggestion $S$ with a function $r(X)$. If $r(X)=1$, we make the display decision using a stage 1 model $m_1(X)$ without generating the suggestion, otherwise if $r(X)=0$ we generate the suggestion $S$ and make the display decision with a stage $2$ model $m_2(X,S)$  as follows: 
\begin{equation}
m(X,S) = r(X) \cdot  m_1(X) + (1-r(X)) \cdot m_2(X,S)
\end{equation}
This formulation allows us to avoid generating suggestions in some cases when we can make an accurate display decision without even knowing the suggestion. For example, in a setting where the programmer has rejected the last 30 suggestions, it is unlikely they would accept the next suggestion. 

\paragraph{Objective and Guarantees.} Our objective to learn the functions $r,m_1,m_2$ is to   1) hide as many  suggestions that would have been rejected  and 2)  maximize the number of display decisions made without generating the suggestion to reduce latency on the system. There is an inherent trade-off between these two objectives as making decisions with access to the suggestions would be more accurate. Moreover, we want to make sure we don't hide suggestions that would have been accepted as this would limit the usefulness of the code assistant. Therefore, we impose a constraint that whenever we hide a suggestion, there is at least a probability $p$ it would have been rejected, a constraint on the  true negative rate (TNR). We translate the objectives and the constraint into the following optimization problem:
\begin{align} \label{eq:cdhf_opt_obj}
& \max_{r,m_1,m_2} \lambda \bE[1 - m(X,S)]  + (1-\lambda) \bE[r(x)] \\ 
& s.t. \ \ \bP(A=\textrm{reject}|m(X,S)=0) \geq p
\end{align}


\paragraph{Parameterization.} We can control the trade-off between the two objectives with a hyperparameter $\lambda \in [0,1]$. Equivalently, instead of controlling the trade-off with $\lambda$, we can set a constraint on $\bE[r(x)]:=R$ and set $\lambda=1$.  We propose an intuitive post-hoc procedure to solve the optimization problem \eqref{eq:cdhf_opt_obj}: we first learn calibrated estimators of the probability of accepting suggestions $\hat{\bP}(A=\textrm{accept}|X,S)$ (with suggestion) and  $\hat{\bP}(A=\textrm{accept}|X)$ (without suggestion). We then parameterize: $$m_1(X)=\bI_{\hat{\bP}(A=\textrm{accept}|X) \geq t_1 }, m_2(X)=\bI_{\hat{\bP}(A=\textrm{accept}|X,S) \geq t_2 }$$ and $r(X) = \bI_{H(\hat{\bP}(A=\textrm{accept}|X)) \leq t_r }$ ($H(.)$ is Shannon's Entropy), and optimize \emph{jointly} over the tuple of thresholds $t_1,t_2,t_r$ over $[0,1]^3$.  This is a fairly efficient procedure that can achieve good results. Two important notes are that this procedure saves latency indirectly by reducing the number of LLM calls across the session and across different users and second, we should still enable the user to see the suggestion with a special keyboard shortcut to override the display decisions. In the next section, we perform a retrospective evaluation of CDHF.

\begin{figure*}[h]
	\centering
	\includegraphics[width=1.0\textwidth]{figures/xgb_features.pdf}
	\caption{Features used to build the action prediction model in our Experiments \ref{sec:experiments}, including from the suggestion, prompt, and session timeline.}
	\label{fig:model_predict}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experiments}\label{sec:experiments}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In these experiments, our main aim is to understand how well our CDHF procedure can make display decisions in a retrospective evaluation. Code is partially available at \footnote{\url{https://github.com/microsoft/coderec_programming_states}} and additional details can be found in the appendix.

\subsection{Dataset and Feature Engineering.}



\paragraph{Dataset.} To build and evaluate our methods, we extract a large number of telemetry logs from \coderec users (mostly software engineers and researchers) in our private organization. Programmers provided consent for the use of their data and its use was approved by our institutional review board. Specifically, for a two-week time period, we extract all the telemetry events for 535 users who code in Python. This totals 4,749 coding sessions, where a session is defined as a continuous sequence of user actions with at most 30 minutes between consecutive events. These sessions are from real-world usage of {\coderec} for daily tasks of the software engineers and researchers, the data was collected prior to the inception of our work. On average each user contributes 9 sessions with each session lasting 21 minutes  (median, 12 minutes). Sessions contain an average of 97 events (show, accept, and reject). This totals to almost 1,675 hours of coding with 168,807 shown events, 
and 33,523 accept events, yielding an acceptance rate of 21.4\% (not meant to represent Copilot average acceptance rate).


\paragraph{Model Features.} The telemetry dataset $D$ described above contains for each user a list of  events in each of their coding sessions, we denote $D_{i,j}$ to be the list of events for the j'th session of the i'th user.  The dataset $\mathbf{D} = \{ D_{i,j} \}$  contains for each user $i$ and session $j$, a list of events occurring in the corresponding coding session. We extract only the accept and reject events, as well as prompt and session features of the corresponding shown events. For each prompt and suggestion pair, we extract: programmer id as one hot vector,
the length of the document, the previous five actions, suggestion features (e.g., suggestion length), previous  features of the last five suggestions shown, the confidence reported by \coderec, an embedding using codeBERTa \cite{feng2020codebert} of prompt and suggestion, presence of Python keywords (e.g., \texttt{import}, \texttt{def}  \texttt{try}, etc.), and the output of the Tree-sitter Parser~\cite{tree_sitter}.
Finally, we extract features of the prompt including its embedding, textual features, and parser outputs.
Figure \ref{fig:model_predict} summarizes the feature engineering. It is crucial to note that the  features do not leak any information about future events and can be computed as soon as a suggestion is generated by {\coderec}. For the first stage model ($m_1$) in CDHFm suggestion features are omitted while we include all features for the second stage model ($m_2$). This feature engineering incorporates past actions and suggestions that the programmer has seen and allows us to use regular ML algorithms instead of time-series methods. 


\subsection{Model Evaluation}
\begin{figure}[h]
    \centering
    \includegraphics[ width=0.7\textwidth]{figures/feat_import.pdf}
    \caption{Feature importance for the seven highest-rated unique features of the model for predicting the likelihood of accepting a suggestion. The feature importance is in terms of the F score which counts how often a feature was split on in the tree ensemble. }
    \label{fig:feature_importance}
\end{figure}
Before we evaluate CDHF, we perform an evaluation of the programmer acceptance model $m_2(X,S)$. We split the telemetry dataset in a 70:10:20 split for training, validation, and testing respectively.  Importantly, we do this split in two ways: 1) by randomly splitting over programmers so that no single programmer is shared across the 3 splits and, 2) by randomly splitting over sessions so that users in training can also be seen in testing to allow for personalization.

\paragraph{Results.} We evaluate different standard machine learning models on this task and find that the best-performing model is eXtreme Gradient Boosting (XGB) \cite{chen2015xgboost}. When we split across users, XGB is able to achieve 81.1\% (95\% CI 80.7-81.6 )  accuracy, and, more importantly, 0.780 (95\% CI 0.775-0.786)  area under the receiver operating characteristic curve (AUC). In the appendix, we show metrics for different models we evaluated including deep networks.
This indicates that the model is able to distinguish between suggestions that are likely to be accepted compared to those likely to be rejected. The model is also well calibrated: the expected calibration error is 0.10 \cite{naeini2015obtaining}. 

\paragraph{Personalization.} We note a significant increase in AUC when we allow for personalization: including programmer ID as a feature and splitting across sessions, this leads to an AUC of 0.795 (95\% CI 0.789-0.801) which is a significant increase (basis of $m_2$ model). When we remove suggestion features from the model, the resulting model (basis of $m_1$ model) achieves an AUC of 0.631 (95\% CI 0.624-0.638). Finally, the time to compute the features needed for the models as well as performing inference on a single data point can take 10ms with a GPU and less than 1ms on a CPU when omitting embeddings, without considering the time to send and receive information from server to client. 


\textbf{Sample Complexity.} To understand how many samples we might need to train individualized CDHF models, we perform a sample complexity analysis on the acceptance prediction stage 2 model where we train with a random fraction of the training dataset in Figure \ref{fig:learning_curveapx}. With 1\% of the training dataset which equates to 1688 training samples, performance reaches 0.69 AU-ROC. With 25\% of training data, the model can achieve 0.75 AU-ROC. 


\begin{figure}[h]
    \centering
    \includegraphics[scale=0.6]{figures/learning_curve.pdf}
        \caption{Sample complexity analysis of the XGBoost stage 2 model when trained on a fraction of the training data and plotting the AU-ROC on the full test set.}
    \label{fig:learning_curveapx}
\end{figure}






\textbf{Factors Influencing Programming Actions.} An analysis of the XGBoost stage 2 model, reveals factors that correlate with programmers' decisions. We examine feature importance weights (Figure \ref{fig:feature_importance}). Specifically, we report feature F-score counts, which capture how often each feature was split in any of the trees in the XGBoost model. The two most important features are the confidence of the suggestion from \coderec's  core suggestion model, and the length of the suggestion. Together, these two features yield a model that achieves an AUROC of 0.71. Other important features include the context of the current event in the coding session such as if the last suggestion was accepted or not. We also see that textual elements of the suggestion are important. For example, the feature indicating if the current suggestion includes the character '\#' (which is used to indicate a comment in Python) was split a total of 8 times. These features should not be interpreted in a causal fashion but rather as being correlated with the behavior of programmers. 






\begin{figure}
	\centering
	\includegraphics[width=0.6\textwidth]{figures/plot_cdhf2023-08-15_182858.pdf}
	\caption{ Evaluation of proposed method CDHF for selectively hiding suggestions. For a given constraint on the FNR in the x-axis (accuracy when a suggestion is hidden), we show on the y-axis the fraction of the total suggestions we can hide while guaranteeing the desired FNR. We plot these curves while varying how often the decision is made generating suggestions (R:=$\bE[r(x)]$, when R=0, we generate the suggestion then decide to hide or not, when R=1, we decide to hide without knowing the suggestion).  }
	\label{fig:cdhf_results}
\end{figure}

\subsection{Retrospective Evaluation of CDHF}


We train the models $m_1$ and $m_2$ using the train set as in the previous subsection. We set the thresholds $t_1,t_2,t_r$ on the validation set for CDHF and evaluate on the test set. 



\paragraph{Results.} In Figure \ref{fig:cdhf_results}, we vary the desired TNR rate (accuracy when a suggestion is hidden) and plot how many suggestions we can hide from those previously displayed while guaranteeing the desired TNR rate. We show the behavior of the CDHF method with different $\lambda$ values, or equivalently with different constraints on how often is the $m_1$ model (first stage) used: $R:=\bE[r(x)]$. To illustrate what our CDHF scheme can accomplish, we can hide 25.3\% of suggestions that were shown while guaranteeing that 94.7\% of them would have been rejected and avoid generating 12.9\% of the suggestions in the first place. If we have no concerns for latency, we can hide 52.9\% of suggestions while guaranteeing that 91.3\% of them would have been rejected. From Figure \ref{fig:cdhf_results}, we can achieve different trade-offs by picking an operating point on any given curve.
Our CDHF procedure is able to satisfy the constraint of FNR  on the test set with a violation of at most 0.3\% i.e. a  guarantee of 95\% FNR on the validation set. equates to 94.7-95.3\% on the test set.


\paragraph{Counterfactual Increase in Acceptance Rate.} On the test set, the acceptance rate of suggestions is 22.5\%. Retrospectively, if we had hidden using CHDF 52.9\% of suggestions, we can compute a counterfactual acceptance rate. The counterfactual acceptance rate can be computed as: $$\frac{\textrm{S accepted} \cdot (1-\textrm{\% hidden} \cdot (1-TNR) )  }{\textrm{S shown} \cdot \textrm{\% not hidden}} = \frac{ 22.5 ( 1-0.529 \cdot 0.087)}{0.471}=45.6\%$$, which is a  23.1 point increase, however, we expect this to be an overestimate.


\paragraph{Discussion and Limitations.} This retrospective evaluation shows that CDHF has promise in reducing developer time spent verifying suggestions or waiting for suggestions. However, our evaluation is retrospective, while GitHub has shown that conditional suggestion filters similar to CDHF increase the acceptance rate of suggestions, a user study evaluation is still required to verify whether it actually makes programmers more productive. As Goodhart's law states that once a metric becomes a target, it ceases to become a good measure, acceptance rate is no exception. Moreover, if CDHF was not properly trained with sufficient data that mimic the programmer's use cases, it might make the programming experience worse by hiding suggestions that are useful.  Moreover, a suggestion that is rejected may still be useful which we do not account for here. Finally, the optimization problem in \eqref{eq:cdhf_opt_obj} is amenable to  procedures inspired  by learning to defer \cite{madras2018predict} that can outperform the post-hoc procedure proposed. 



\section{Which Suggestion to Show?}

In this paper, we primarily focused on  the design problem of when to display suggestions and did not tackle the question of which suggestions to display among a candidate set. Given access to telemetry data, which consists of contextualized suggestions with either accept or reject signals, one can interpret an accept as the act of preferring a suggestion over no suggestion. Thus, it is reasonable to think one can use the telemetry data as a sort of preference dataset and build a reward model of the programmer preference which would in short be equivalent to estimating the programmer acceptance probability $\hat{\bP}(A=\textrm{accept}|X,S)$. Therefore, a reasonable procedure would be to take a candidate set of suggestions $\mathcal{S}$ and display the suggestion that maximizes the probability of acceptance in the set; this is essentially the best-of-$n$ baseline in RLHF \cite{rafailov2023direct}.

\paragraph{Potential Bias Towards Short Suggestions.} However, we hypothesize that such a ranking scheme would not be  productive and  can lead to worse suggestions of short length. Our rationale is the following: suppose the LLM is able to generate a multi-line suggestion $S$ for a user query that approximately matches what the user desires. To maximize the probability that the user accepts the suggestion, it would be advantageous to split the suggestion $S$ line-by-line and display it to the user step-by-step. The reasoning is that it is more likely for the first line of $S$ to be correct rather than all of $S$ being correct, hence being more likely to be accepted.




\paragraph{Experiment.} To test this hypothesis, we perform the following experiment: we learn a model $m$ of suggestion acceptance given only the prompt and suggestion embeddings with no session features on the telemetry data from the previous section. We then leverage the HumanEval dataset \cite{chen2021evaluating} which consists of 164 Python problems each with an associated docstring and a ground truth function body solution - solutions have at least 2 lines and 7 median lines of code. Given the model $m$ and each problem, we let the prompt be the concatenation of the docstring and the first $k$ lines of the solution and let the candidate set of suggestions $\mathcal{S}$ be as follows: given the solution $S$ represented as an array of tokens of length $N$, we let $\mathcal{S}=\{S[:i]\}_{i=1}^{N}$. For example, if the solution $S$ was "return np.mean(x)", then $\mathcal{S}=\{\textrm{"return"},\textrm{"return np.mean(x)"} \}$.

\paragraph{Results.} We vary the parameter $k$ in the set $\{0,1,2,3\}$ so that prompt goes from the docstring to include lines of the solution. When $k=0$, the normalized length of the highest-rated suggestion according to the model across the 164 problems is almost uniform across $[0,1]$, a Kolmogorov–Smirnov test compared to the uniform distribution has a p-value of 0.53 (KS=0.06). 
Optimally we want the normalized length to cluster around $1$ to include the full solution. However, when $k>0$, meaning that the prompt includes lines of code, we find that for over 60 of the 164 problems, the highest-scored suggestion lies in $[0,0.2]$, and for at least 40 problems it is the first token. A histogram showing this phenomenon is in Figure \ref{fig:which_k1} for $k=1$.  This provides some evidence that optimizing for acceptance can have a bias toward shorter suggestions since the highest-ranked suggestion is often in first few lines of the solution.

\paragraph{Limitations.} However, there are important limitations in our experiment. First of all, the model $m$ is only trained on Copilot suggestion, thus the bias towards short suggestions can be partially due to Copilot potentially showing short suggestions. In that case, we can at least say that maximizing accepts would not elevate that problem. Second
we used embeddings of the suggestions for the reward model which while accurately predictive of accepts (AUC=0.701) might be biased in some ways compared to fine-tuning the language model.


\begin{figure}[H]
  \centering
  \subfigure[Histogram of position of max suggestion]{
    \includegraphics[width=0.45\textwidth]{figures/histogram_maxindex_1.pdf}
    \label{fig:plot1}
  }
  \hfill
  \subfigure[Probability of acceptance by length]{
    \includegraphics[width=0.45\textwidth]{figures/plot_score_trend_1.pdf}
    \label{fig:plot2}
  }
  \caption{Plots for the experiment on ranking suggestions by the probability of acceptance. Histogram (a) shows in which length percentile bin the suggestion maximizing the probability of acceptance lies and Graph (b) shows the acceptance score by increasing the length of the suggestion. These plots are for $k=1$ (docstring + first line of solution) }
  \label{fig:which_k1}
\end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusion}\label{sec:conclusion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We proposed a strategy to decide when to display code suggestions in AI-assisted programming to improve time efficiency. This strategy was based on a utility theory formulation and employs a two-stage procedure using a predictive model of suggestion acceptance. A retrospective evaluation showed that we can reduce the number of suggestions and thus programmers' time without sacrificing the utility of \coderec. However, a prospective study that evaluates the impact of \coderec with and without CDHF could help with conclusive evaluation and is the basis of future work. Moreover, future work will attempt to directly estimate Proposition 1 leveraging improved methods. We don't believe that CDHF can introduce negative consequences beyond what \coderec introduces to the programmer as it functions as a filtering mechanism for unhelpful suggestions. Moreover, we believe that the CDHF methodology can be employed in a wide range of streaming human-AI collaboration tasks such as assisted writing. Future work will incorporate the latent state of the programmer into the predictive models by leveraging data modalities beyond telemetry and investigating other signals beyond acceptance of suggestions to improve the underlying LLM.


\section*{Acknowledgments}

HM partly conducted this work during an internship at Microsoft Research (MSR). We acknowledge valuable feedback from colleagues across MSR and GitHub including Saleema Amershi, Victor Dibia, Forough Poursabzi, Andrew Rice, Eirini Kalliamvakou, and Edward Aftandilian.

